Deeper Thought, Weaker Aim: Understanding and Mitigating Perceptual Impairment during Reasoning in Multimodal Large Language Models

Multimodal large language models (MLLMs) often suffer from perceptual impairments under extended reasoning modes, particularly in visual question answering (VQA) tasks. We identify attention dispersion as the underlying cause: during multi-step reasoning, the model's visual attention becomes scattered and drifts away from question-relevant regions, effectively "losing focus" on the visual input. To better understand this phenomenon, we analyze the attention maps of MLLMs and observe that reasoning prompts significantly reduce attention to regions critical for answering the question. We further find a strong correlation between the model's overall attention on image tokens and the spatial dispersiveness of its attention within the image. Leveraging this insight, we propose a training-free Visual Region-Guided Attention (VRGA) framework that selects visual heads based on an entropy-focus criterion and reweights their attention, effectively guiding the model to focus on question-relevant regions during reasoning. Extensive experiments on vision-language benchmarks demonstrate that our method effectively alleviates perceptual degradation, leading to improvements in visual grounding and reasoning accuracy while providing interpretable insights into how MLLMs process visual information.

==> data/a.tex <==
Step   1: loss=0.80732453, grad_norm=0.228018
Step  11: loss=1.24353981, grad_norm=0.999999
Step  21: loss=1.71383822, grad_norm=0.531556
Step  31: loss=1.26907802, grad_norm=0.479314
Step  41: loss=0.61436760, grad_norm=0.223428
Step  51: loss=0.65446341, grad_norm=0.605004
Step  61: loss=1.15822339, grad_norm=0.447390
Step  71: loss=1.22236466, grad_norm=0.477490
Step  81: loss=0.94669211, grad_norm=0.963342
Step  91: loss=0.96946740, grad_norm=0.251855
Step 100: loss=1.35207486, grad_norm=0.973686

======================================================================
训练完成
======================================================================

✅ 结果已保存到: complex_attention_20260326_154631.json

======================================================================
训练关键统计
======================================================================
初始Loss (step 0):  0.8073245287
最终Loss (step 99): 1.3520748615
Loss下降: -0.544750
初始梯度范数: 0.228018
最终梯度范数: 0.973686

第一个Attention Block的注意力权重均值:
  初始: 0.020000
  最终: 0.020000

�� 用于对比的哈希值:
  轻量级哈希 (loss+grad_norm): 091223c4e2bf5dfd3334f87b581355ff
  完整哈希 (所有梯度采样): 072f0ac717f54c37e0885a0581c9632e...

======================================================================


"""
测试GPU vs CPU差异 - 禁用归一化层
文件名: debug_attention_no_norm.py
"""

import torch
import torch.nn as nn
import torch.nn.functional as F
import json
import hashlib
from datetime import datetime

# 设置确定性
torch.backends.cudnn.deterministic = True
torch.backends.cudnn.benchmark = False
torch.manual_seed(42)

if torch.cuda.is_available():
    torch.cuda.manual_seed_all(42)

class SimpleTransformerNoNorm(nn.Module):
    """移除BatchNorm和Dropout的版本"""
    def __init__(self):
        super().__init__()
        self.embed = nn.Linear(100, 128)
        self.attention = nn.MultiheadAttention(128, num_heads=8, batch_first=True)
        # 移除LayerNorm
        # self.norm1 = nn.LayerNorm(128)
        # self.norm2 = nn.LayerNorm(128)
        self.ffn = nn.Sequential(
            nn.Linear(128, 512),
            nn.GELU(),
            nn.Linear(512, 128)
        )
        self.fc = nn.Linear(128, 1)
        
    def forward(self, x):
        x = self.embed(x)
        attn_out, attn_weights = self.attention(x, x, x)
        x = x + attn_out  # 直接残差连接，无Norm
        ffn_out = self.ffn(x)
        x = x + ffn_out  # 直接残差连接，无Norm
        x = x.mean(dim=1)
        return self.fc(x), attn_weights

# 测试GPU和CPU
def test_on_device(device):
    print(f"\n{'='*50}")
    print(f"测试设备: {device}")
    print('='*50)
    
    model = SimpleTransformerNoNorm().to(device)
    optimizer = torch.optim.Adam(model.parameters(), lr=0.001)
    
    torch.manual_seed(42)
    X_fixed = torch.randn(500, 20, 100)
    Y_fixed = torch.randn(500, 1)
    
    losses = []
    for step in range(100):
        batch_size = 16
        idx = (step * batch_size) % 500
        x = X_fixed[idx:idx+batch_size].to(device)
        y = Y_fixed[idx:idx+batch_size].to(device)
        
        optimizer.zero_grad()
        output, _ = model(x)
        loss = F.mse_loss(output, y)
        loss.backward()
        optimizer.step()
        
        losses.append(loss.item())
        
        if step % 10 == 0:
            print(f"  Step {step+1:3d}: loss={loss.item():.8f}")
    
    return losses

# 运行测试
print("测试移除BatchNorm和Dropout后的模型")
cpu_losses = test_on_device('cpu')
if torch.cuda.is_available():
    gpu_losses = test_on_device('cuda')
    
    # 对比结果
    print("\n" + "="*50)
    print("对比结果")
    print("="*50)
    print(f"CPU 最终Loss: {cpu_losses[-1]:.8f}")
    print(f"GPU 最终Loss: {gpu_losses[-1]:.8f}")
    print(f"差异: {abs(cpu_losses[-1] - gpu_losses[-1]):.2e}")
    
    if abs(cpu_losses[-1] - gpu_losses[-1]) < 1e-5:
        print("✅ 移除归一化层后，GPU和CPU结果一致！")
        print("问题出在BatchNorm或Dropout上")
    else:
        print("⚠️ 仍然存在差异，需要进一步排查")

==> data/b.tex <==
import torch
import torch.nn as nn
import torch.nn.functional as F
import copy

# ====== config ======
torch.manual_seed(0)
torch.cuda.manual_seed_all(0)

torch.backends.cuda.matmul.allow_tf32 = False
torch.backends.cudnn.allow_tf32 = False

# ====== model ======
class Block(nn.Module):
    def __init__(self, dim=64, heads=4):
        super().__init__()
        self.attn = nn.MultiheadAttention(dim, heads, batch_first=True)
        self.mlp = nn.Sequential(
            nn.Linear(dim, dim * 4),
            nn.ReLU(),
            nn.Linear(dim * 4, dim)
        )
        self.ln1 = nn.LayerNorm(dim)
        self.ln2 = nn.LayerNorm(dim)

    def forward(self, x):
        a, _ = self.attn(x, x, x)
        x = x + a
        x = self.ln1(x)

        m = self.mlp(x)
        x = x + m
        x = self.ln2(x)
        return x


class ToyTransformer(nn.Module):
    def __init__(self, depth=6, dim=64):
        super().__init__()
        self.blocks = nn.ModuleList([Block(dim) for _ in range(depth)])
        self.head = nn.Linear(dim, dim)

    def forward(self, x):
        for blk in self.blocks:
            x = blk(x)
        return self.head(x)


# ====== divergence test ======
def run(seed_shift=0):
    torch.manual_seed(0 + seed_shift)
    torch.cuda.manual_seed_all(0 + seed_shift)

    model = ToyTransformer().cuda()
    opt = torch.optim.AdamW(model.parameters(), lr=1e-3)

    x = torch.randn(2, 16, 64).cuda()
    target = torch.zeros_like(x)

    traj = []

    for step in range(50):
        opt.zero_grad()
        out = model(x)
        loss = F.mse_loss(out, target)
        loss.backward()
        opt.step()

        traj.append(out.detach().cpu())

    return traj


# ====== compare two runs ======
traj1 = run(seed_shift=0)
traj2 = run(seed_shift=0)  # 理论上应该一样

for i in range(len(traj1)):
    diff = (traj1[i] - traj2[i]).abs().max().item()
    print(f"Step {i}: diff = {diff:.6e}")
